Information Retrieval for ZeroSpeech 2021: The Submission by University of Wroclaw

We present a number of low-resource approaches to the tasks of the Zero Resource Speech Challenge 2021. We build on the unsupervised representations of speech proposed by the organizers as a baseline, derived from CPC and clustered with the k-means algorithm. We demonstrate that simple methods of refining those representations can narrow the gap, or even improve upon the solutions which use a high computational budget. The results lead to the conclusion that the CPC-derived representations are still too noisy for training language models, but stable enough for simpler forms of pattern matching and retrieval.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> LaTeX/old_simi.tex <==
\section{Semantic task: sSIMI}
\todo[inline]{A short description of the task (say that there are multiple audio files for a single word). -- maybe not needed}

 The submission format encouraged solutions, which assign a vector at every temporal location, and a pooling method to aggregate them into a vector for the recording.
The similarity measure for such recording vectors had to be chosen from metrics
supported by scipy.spatial.distance.cdist (for instance cosine, or euclidean). Then the correlation between these distances and human semantic similarity judgements are computed .
% 2. Our assumptions

Consider a more general problem -
building word representations to approximate human semantic similarity judgments -
with fairly unconstrained resources and modalities.
A straightforward approach would be to collect a large corpora of text,
and train context-less word embeddings~\cite{}.  % -- if possible, reference not w2v but a paper which shows approximation to human-judged similarity 

In contrast, the ZeroSpeech semantic similarity task imposes additional constraints: the data is provided in form of recordings, the training set is small and not segmented into words. We opted for using the outlined solution, and address the aforementioned problems one by one.\\

\noindent\textbf{Preparation of the Corpora} We rely on the baseline pseudo-phoneme units, extracted with CPC and quantized with k-Means. Given a perfect mapping of pseudo-phones to actual phones, such units are correct on ca. $42\%$ of positions. Note that for our solution, we never need to explicitly build such mapping.

A recognized stream of pseudo-phones for a given utterance, for instance
%
\begin{center}
\texttt{31,12,12,12,13,13,13,13,13,13,8,8,8,8}
\end{center}
%
differs from a regular text, by adding the temporal quality: some phones form long strings of repeated tokens, and phone boundaries tend to be noisy. 
First of all (jakos ladniej) we treat the signal as a sequence of blocks:

31 $\times$ 1, 12$\times$3, 13$\times$6, $8\times4$

We tested two different approaches: in the first, low-level one use the above blocks as atoms, and treat signal as a sequence of such atoms. In the second we try to use these blocks to form larger units (hopefully corresponding to words, or to word-pieces\cite{})\\

\noindent\textbf{Pseudophoneme approach}
For the whole quantized librispeech we compute block embeddings using Word2Vec (with a small window, since we need rather syntactic than semantic embeddings). We obtain NNN 100-dimentional vectors corresponding to different blocks (on average N length variants per one cluster). Note, that since Word2Vec is also a language model, our approach can be treated as a super-simplification of a baseline ZeroSpeech models, where embeddings are context-free and instead of LSTM or BERT we use a skip-gram based neural language model.

Having these embedding we can obtain the vector for every utterannce just by taking the average of vectors of its blocks. Since our vectors are utterance oriented we have to repeat it for every sequence element (and use any pooling procedure to obtains the final vector)\\

\noindent\textbf{Pseudoword approach}
We attempt to removing the temporal quality by heuristically processing such strings (e.g., collapsing subsequent streams of tokens).

\todo[inline]{Describe in detail.}

% 3. The solution
\noindent\textbf{Segmentation}
We apply segmentation into pseudo-words with the method based on a unigram language model\cite{kudo_subword_2018}. Given a vocabulary $\mathcal{V}={w_1,\ldots,w_n}$ with associated occurrence probabilities $(p_1,\ldots,p_n)$, a utterance $x$, the most probable segmentation is determined with the Viterbi algorithm.
The vocabulary $\mathcal{V}$ is refined iteratively, by maximizing the probability of every utterance under a unigram language model:
\begin{equation}
    P(x) = \prod_i p(x_i).
\end{equation}
To this end, we use SentencePiece~\cite{kudo_sentencepiece_2018} with target vocabulary size \todo{Vocab size? 50K}. Figure~\ref{fig:sentpieces} presents samples from vocabularies trained on ground truth transcriptions, and on CPC--K-Means cluster ids translated to phonemes with ground truth alignments. \todo[inline]{A smart comment, e.g., we dont care about "iwantto" being glued together, etc.}

\noindent\textbf{Embedding and Retrieval}
Having a training corpora split into pseudo-words, we train ordinary word2vec~\cite{}. The corpora has XXX words with an average length XXX (
\todo[inline]{A small summary - \# of words, avg word len of gt transcripts, gt transcripts sentencepieced, and our pseudo-word-sentencepieces?}

When processing the recordings from the ZeroSpeech similarity task, we convert them to psuedo-phones with the same CPC--K-Means model, and process heuristically.
Because the recordings are of individual words, no segmentation is necessary, but the pseudo-words may not exist in the vocabulary. Instead of segmenting them with SentencePiece, we find the closest matches in the training set wrt. edit distance, and then average word2vec embeddings of these. We return a single embedding for every input phrase.


\subsection{SIMI. Experiments}

Since our approach differs from the one suggested in the ZeroSpeech contest we decide to present other word oriented toplines for SIMI (following our ideas). We consider downloaded vectors trained on a large corpora (\ref{}), embedings trained on LisbriSpeech transcriptions and embeddings trained on our tokenization of librispeech transcription (in the last case we deleted spaces and found 50K tokens using SentencePiece). Results are presented in Table \ref{}). As one can see embedings trained on word corporas outperform Roberta topline, which can be treated as [że warto w tę stronę iść, jakoś zgrabnie napisać]


\begin{table}[htb]
  \centering
  \caption{Toplines for word based SIMI (all results on dev set)}
  \label{tab:simi_toplines}
  \begin{tabular}{l|l|l}  
    \toprule
  \textbf{Method}                      & synth. & libri \\ \hline  
  Google News Word2Vec                 & 65.5   &  \\ \hline
  LibriSpeech 960 transcriptions (w2v) & 36.3   &  \\ \hline
  Tokenized Librispeech                & 16.8  &   \\ \hline
  RoBERTa (ZS Topline)                 &        &
 \end{tabular}
\end{table}

Table \ref{} shows our results in the ZeroSpeech contest (together with other submissions). It's worth to stress that phoneme approach works fine on LibriSpeech part of the data [but in general all results are not very far from the noice] 

